Interactive Visual Study of Multiple Attributes Learning Model of X-Ray Scattering Images

Existing interactive visualization tools for deep learning are mostly applied to the training, debugging, and refinement of neural network models working on natural images. However, visual analytics tools are lacking for the specific application of x-ray image classification with multiple structural attributes. In this paper, we present an interactive system for domain scientists to visually study the multiple attributes learning models applied to x-ray scattering images. It allows domain scientists to interactively explore this important type of scientific images in embedded spaces that are defined on the model prediction output, the actual labels, and the discovered feature space of neural networks. Users are allowed to flexibly select instance images, their clusters, and compare them regarding the specified visual representation of attributes. The exploration is guided by the manifestation of model performance related to mutual relationships among attributes, which often affect the learning accuracy and effectiveness. The system thus supports domain scientists to improve the training dataset and model, find questionable attributes labels, and identify outlier images or spurious data clusters. Case studies and scientists feedback demonstrate its functionalities and usefulness.

==> README <==
Created by Torsten Moeller (vis@cs.sfu.ca), April 6 2004
modified by Steven Bergner and Torsten Moeller, June 30 2006
modified by James Peltier and Torsten Moeller, March 28, 2007
modified by Bernhard Finkbeiner, July 5, 2010
modified by Tobias Isenberg, January 2016
modified by Filip Sadlo, March 2016
modified by Tobias Isenberg, July 2016

This distribution provides a document class for formatting papers according to the specifications for submission to conferences sponsored by the IEEE Visualization & Graphics Technical Committee (VGTC).

Conferences that use the 'journal' document option:
- IEEE Visualization Conference (VIS, incl. InfoVis, SciVis, VAST)
- IEEE Virtual Reality (VR)
- IEEE International Symposium on Mixed and Augmented Reality (ISMAR)

It contains 13 files/directories:

README          - this file
diamondrule.eps - abstract and body separator
diamondrule.pdf - its PDF version
vgtc.cls        - the VGTC class file, which should be placed, somewhere in the TeX search path (or in the local directory)
template.tex    - an example paper
template.bib    - a small bibliography file used by the example
template.pdf    - an example proper pdf output in default journal mode
abbrv-doi*.bst  - four different versions to generate the bibliography including DOI output, with and without hyperref support, with and without narrow rendering of DOIs
makefile        - makefile including bibtex compilation and proper PDF generation
pictures/       - subdirectory with sample images, both in EPS and in direct pixel/vector format

Usage
=====

The template can be used as such (using the established LaTeX environments) by calling pdfLaTeX or LaTex. For Windows-based LaTeX installations you can use, for example, the environment provided by http://www.texniccenter.org/ along with MikTeX (http://miktex.org/). For Uinux-based installations, please use your favorite LaTeX distribution and editing environment or use the makefile following the instructions below.

Use of the Makefile
===================

Prior to "building" a paper please be sure to run

  make clean

This will ensure that the paper is built cleanly each and every time. We suggest to run this command before each new compilation.

To compile the example, run

  make

or manually, if the makefile does not work for you

  latex template
  bibtex template
  latex template
  latex template

If you run 'make' for the first time, a successful compilation will create a file called 'template.pdf'. Please make sure, that its layout is identical to the file 'template-journal.pdf' provided with this package.

The included makefile also allows you to run each step of the process manually.  Below are a list of available options that may be passed to make

 "make clean"
   removes all files that can be generated automatically.

 "make gs7"
   This will perform all functions to build a proper paper using GhostScript 7.

 "make gs8"
   This will perform all functions to build a proper paper using GhostScript 8.

 "make dvi"
   This will process the .tex file and produce a DVI output file.  This
   step may process the .tex file several times to process all references
   and citations.

 "make ps"
   This will process the .tex file and the DVI output and convert it to a
   PostScript file.

 "make pdf"
   This will process the .tex file using pdfTeX/pdflatex to produce a PDF
   file directly (not using a DVI and PostScript file).
   Please make sure that all fonts are embedded.
   You can use pdffonts my_document.pdf to check if they are.
   It is standard in all modern latex distributions.
   If you use eps figures (e.g. R or gnuplot figures) which you convert to
   PDF using epstopdf, do the following:
   Use GL_OPTIONS, a global environment variable for ghostscript:
   export GS_OPTIONS="-dEmbedAllFonts=true -dPDFSETTINGS=/printer"
   # and run
   epstopdf myfile.eps

   See http://bugs.debian.org/cgi-bin/bugreport.cgi?bug=411651 for the
   origin of this solution.


If you have problems with the makefile please notify us with the output of
the errors produced when running make and we will work to figure out the
resolution.


To produce proper pdf output, please use:
  dvips -t letter -Pdownload35 -Ppdf -G0 template.dvi -o template.ps

The "-Ppdf" and "-G0" flags should be specified in that order; reversing
them does not work, and will result in unacceptable results.

The following information is an exerpt from the ACM SIGGRAPH Conference /
Symposium / Workshop Content Formatting Instructions which can be found
here.

 http://www.siggraph.org/publications/instructions/author-instructions.pdf

If you are using version 7.x of GhostScript, please use the following
method of invoking ‘ps2pdf,’ in order to embed all typefaces and ensure
that images are not downsampled or subsampled in the PDF creation process:

 ps2pdf -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 \
        -dSubsetFonts=true -dEmbedAllFonts=true \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

If you are using version 8.x of GhostScript, please use this method in
place of the example above:

 ps2pdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.3 \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

This has been incorporated into the makefile and should no longer be needed
unless you are building the PDF file manually.


==> makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = template.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = template.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< template.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)


==> sections_version_old/casestudy.tex <==
\section{Case Studies}
We have conducted several case studies with domain scientists to show the usability of the \hl{visualization system}.

\begin{figure*}[t]
 \centering
 \includegraphics[width=\textwidth]{images/CaseRings.png}
    \caption{ Studying two groups of images where attributes ``Many rings'', ``Ring'', and ``Strong scattering'' co-exist. (G1) ``Many rings'' are not detected; (G2) ``Strong scattering'' are not detected. The image thumbnail galleries and the FEA embedded space are shown, together with detail view of several images.}\vspace{-5pt} 
    \label{fig_CaseRings} 
\end{figure*}

\subsection{Case 1: Studying model performance from an ACT image group}

Fig. \ref{fig_interface} shows an image group (in blue dots) selected from ACT space, based on high prediction error rate (the dots with higher opacity). These images are the most problematic candidates. By putting this selection into the group panel, the measures view \hl{ (Fig.} \ref{fig:PCP}\hl{)} indicates that a structural attribute ``Linear beamstop'' is the most important in this group. \hl{Switching to the clustering view in} Fig. \ref{fig_interface}(F1), the images form two spatial clusters in PRD space. The red petal of the attribute flowers indicates ``Linear beamstop''. In the bottom cluster, images with this attribute are predicted correctly such as Image 54, 62 and 139. From the detail view (Fig.\ref{fig_interface}(G)), the three images are very different (Image 62 has a blue background and needle shape under the beam) while the learning model gives correct prediction on this attribute. 

However, most images in the top cluster of Fig. \ref{fig_interface}(F1) are wrongly classified. For example, Images 44, 38, and 4 fail the detection of linear beamstop. Instead, they are detected as other types of beam stops: ``Wedge Beamstop'' or ``Circular Beamstop''. Referring to the Fig. \ref{fig:matrix},  the coefficients of correlation matrix between any pair of these three different beamstops are negative, telling they are negatively dependent and exclusive to each other in an image. The conditional entropy  between them in the green true space are zero, which further verifies they are exclusionary. But the conditional entropy values for these pairs in the blue prediction space are non-zero values. Thus, it shows the model cannot tell the differences of the three different beamstop attributes.  

By further putting this group into Fig. \ref{fig_interface}(F2) and using FEA space instead with 2 spatial clusters, Images 44, 38, 4, and 139 are close together. The convolutional part of the network finds they have similar high-level image features. But the fully connected classifier may be confused and give different predictions of beam stop types. This shows that the x-ray scattering attributes of different types of beam stops are quite hard to detect due to the small size and especially with dark black background. Therefore, the \hl{visualization system} helps scientists recognize the weak point of a learning model, which may be addressed by further extending the convolutional layers and training the model with more images to distinguish them in the feature space. 

\subsection{Case 2: Studying model behavior with three co-existence attributes}

From the 3-attribute co-existence table of Fig. \ref{fig:coexistencetable}, three attributes of interest are identified: ``Many rings'', ``Ring'', and ``Strong scattering''. These attributes are highly correlated and scientists want to confirm how the network distinguish them. In the dataset, there are totally 54 images sharing the attributes which are correctly detected in 34 images. By selecting these attributes, from the attribute set view of Fig. \ref{fig:attributepanel}, users can identify different combinations and find the model output of them. For example, two combinations are selected to groups of interest: (G1) six images where ``Many rings'' are not detected; (G2) three images where ``Strong scattering'' are not detected. The two selections are put into the group panel for comparison, as shown in Fig. \ref{fig_CaseRings}. Here the thumbnail galleries of them are shown. Note that all the images have the attribute ``Ring'' detected correctly while their visual appearances are quite diverse, where the high variation of x-scattering structures are manifested. 

In the embedded view of FEA space, G1 images are shown in blue dots and G2 images are in green dots (the color can be selected by users flexibly). It can be seen that G2 images are far away from each other. But Image 77 in G2 are very close to Images 80 and 296 in G1 (see the pink circle). When opened in the detail view, the three images have similar features of rings whose center roughly lies on edges and corners. The model detects many rings in Image 77 but not in Image 296. It helps scientists to identify that the model does not perform as expected for ``Many rings'' due to the fact that the rings in Image 296 is not as complete as in Image 77. Here, since high-level FEA features are extracted correctly, to improve the model, the fully-connected layers may be replaced with other classifiers (e.g., Support-Vector Machine).

In G1 images, 183, 112, and 132 are close in FEA space (see the blue circle). In detail view (first three images), they have specular backgrounds with strong scattering (which is related with bragg angle of light beams). The ``many rings'' structure is quite hard to discern from low-level pixel-based metrics. This type of ``Many rings'' may need to be labelled in a separate way, which suggests scientists to use a refined attribute list in sufficiently describing the image structures.

\subsection{Case 3: Studying the pre-trained model error}

\begin{figure*}[t]\centering
 \includegraphics[width=\textwidth]{images/case3_updated.png}
    \caption{ Debugging the issue of the pre-trained ResNet model for two attributes BCC and FCC through the entire visualization elements. }
    \label{fig:Debug_case} 
\end{figure*}

By exploring the co-existence matrices in Fig. \ref{fig:matrix}, we notice that two attributes  ``BCC'' (body-centered cubic) and  ``FCC'' (face-centered cubic) are presented as anomalies. For example, in the correlation matrix (the top one in the figure), the values paired with ``BCC'' in PRD space are zero, which are inconsistent with the values in ACT space. The other attribute ``FCC'' is similar. Moreover, the conditional entropy in ACT space (the bottom matrix in the figure) for the two attributes present normal relationships with other attributes. Both observations indicate the predictions by the pre-trained model are erroneous for these two attributes.

As shown in Fig. \ref{fig:Debug_case}, we study the two attributes by filtering out all others labels in the attributes list. In the ACT space, three clusters are formed that are highlighted in blue, purple, and green (highlighted in orange box), correspondingly. They represent the image clusters with only ``BCC'', only ``FCC'', and both attributes, respectively. These two attributes describe the feature of crystal structures. Typically, since the atoms in a unit cell can only form one structure, the two structures are mutually exclusive to each other. But some material sample can have two structure units superimposed. Therefore, the six abnormal image points, shown as a small group in the orange box of ACT space, are identified. 

Next, we examine the two dense clusters in blue and purple colors in ACT space to learn more details. These two attributes cannot be separated well in both FEA and PRD spaces. As shown in Fig. \ref{fig:Debug_case}, the image points with purple and blue colors are mixed in the two embedded visualizations. %It is probably rooted in the pre-trained model, either not trained well or the two attributes can hardly be distinguished, so that both the generated feature vector and the prediction vector are not sufficient to describe their difference. 

To find out the reason, we check the performance of the two groups by looking into the parallel coordinates in the group panel (in the middle of Fig. \ref{fig:Debug_case}). First, Selection 1 (the blue cluster in ACT space) shows that all 247 images in this selection with attribute  ``BCC'' have zero true positive and zero true negative. The accuracy, precision, and recall are all zeros and F1 score shows NaN for  ``BCC''. It means the model is unable to predict the ``BCC'' attribute. At the same time, we find the model does not confuse the  ``BCC'' attribute to  ``FCC'', since this group has all images predicted true negative for ``FCC''. So it has a good accuracy value 1 for  ``FCC'' prediction. In Selection 2, the situation for attribute  ``BCC'' and  ``FCC'' in parallel coordinate curves is the same as in Selection 1. Both of these indicate that the ResNet model does not successfully classify these two attributes. The possible reason could be: 1) insufficient data labeled with these attributes in the training set; 2) the feature of these attributes are too similar to distinguish; or 3) they are affected and overwritten by other strong signal attributes. 

To further check the reason, we click on some of the images from the two groups to observe their original x-ray images, as shown in the image view at the bottom of Fig. \ref{fig:Debug_case}. The  ``BCC'' and ``FCC'' attributes can be found by domain scientists on the colorful spots with periodical intensity variation on the rings. They are not suppressed by other attributes like "many rings". We also find that a quite small number of images with these two attributes were used in model training. Finally, we check the model implementation and identify an error in the data processing function that learned incorrect names for the two attributes. This example shows the \hl{visualization system} helps users discover mistakes or errors in modeling.

==> sections_version_old/conclusion.tex <==
\section{Conclusion and Future Work}
We present a visual system for understanding the learning model of x-scattering images with multiple attributes. The system allows users to visually discover the embedded distributions of feature vectors, predictions, and actual labels of these images. User interactions are supported to compare selected instance images and study their prediction results related to the attributes \hl{to understand the behavior of pretrained model. The current limitation of the system is that it did not integrate the training process and mount its direct trained model together with test image dataset as the input to the system yet.} In future work, we will \hl{integrate the visualization analysis into the training process and} extend the work for model debugging and refinement, by taking neurons and different network layers into account, so as to study how they relate to the prediction of multiple attributes. 

==> sections_version_old/design.tex <==
\section{Design of the Visualization System}

\subsection{Analysis Task Characterization} 
Domain scientists currently often use the statistical metrics such as precision, recall and AP for learning model evaluation of x-ray scattering images. However, it can hardly help scientists explain and make sense of how the model performs on specific images with various structural patterns. Visual analytics tools can play an important role for model understanding through interactive visualizations directly over images and attributes. We conducted a requirement analysis with material scientists who want to understand the ResNet model behavior over the x-ray scattering image dataset, which defines the visual analysis tasks listed below. 

    \noindent \textbf{T1. Analysis in Model Spaces:} Investigate scientific images within the spaces of ACT, PRD and FEA, for users to understand how the images are modelled by the ResNet in the feature space and then classified by fully connected layers in the prediction space, with respect to the real labels.\\
    \noindent \textbf{T2. Analysis with Group Behaviors:} Examine specific groups of images in the ACT, PRD and FEA spaces, in order to find important clusters and outliers. \\
    \noindent \textbf{T3. Analysis with Image Attributes:} Identify important image instances with the performance metrics of individual attributes and co-existent attributes to perform the first two tasks. \\
    \noindent \textbf{T4. Analysis with Comparisons:} Compare individual images and image clusters for the model prediction performance.
    
\st{The current focus in this paper is to study the prediction results and understand the behavior of ResNet model. The scientists are also interested in visualization tools to be integrated within the training process, for model debugging and refinement, which will be addressed in our future work.}


\subsection{Visualization Design and Interface Overview} 
With respect to these tasks, we design the \hl{visualization system} by integrating a set of visual interaction functions  including:
\begin{itemize}   
\item {\bf For T1: Coordinated Visualization in Embedded Spaces:} Images are visualized in the 2D canvases of ACT, PRD and FEA spaces, respectively, where a t-SNE algorithm is adopted to project them onto the 2D spaces by the corresponding vectors. Users can select images and image groups interactively, and then discover their distribution within different spaces.

\item {\bf For T2: Image Group Selection and Visualization:} 
Users can group images into selections from each embedded space by lasso tools. The images in each group are visualized by an embedded view from one of the three spaces, a statistic view of image metrics, and an image gallery view. The selections can be studied in group panels where they can be further clustered by the model performance measures for drill-down study and comparison. 

\item {\bf For T3: Attribute Co-existence Visualization:} The model performance with co-existence attribute relations are visualized in an interactive view. Users can then define image groups based on the visual cues of model performance. 

\item {\bf For T4. Group Comparative View and Image Comparison:} The selected groups can be easily investigated and compared with group panels for detail views. Through interactive selection over all the above visualizations, users can also open multiple images to compare their details of raw data and model predictions.
\end{itemize}

Fig. \ref{fig_interface} shows the \hl{visualization system} interface. It displays the scientific images in the coordinated views (C)-(E) of three different embedded spaces (ACT, FEA, PRD). Users can interactively select (with zooming, panning, and lasso-selection) image groups in either embedded view, which is highlighted to show their distributions in the other views. Each image in the embedded space can be shown as dots (C)-(E) whose transparency indicates model predicted errors. Users can filter the visualizations with single or multiple attributes (B). Moreover, the co-existence measures provide visual cues for attributes combinations of interest. Users can study multiple selected group in the group panels (F1 and F2), where they can also compare them. In each panel, three tab views can be switched to visualize: (1) attribute measures as parallel coordinates plots (see Fig. \ref{fig:PCP}) including as TP, TN, FP, FN and accuracy, precision, etc.; (2) image clusters (F1) and (F2) based on their distance in different data spaces; (3) image thumbnails (See Fig. \ref{fig_CaseRings}). All these views are coordinated for synchronized changes. Clicking any image instance also adds it to a detail image view (G). The attribute values of actual labels and predicted labels are visualized. Next we discuss details about visual exploration with these views.

\subsection{Image Exploration in Embedded Spaces}

When a set of x-ray scattering images are loaded into the system, the corresponding structural attributes are loaded and shown in the attribute panel (Fig. \ref{fig_interface}B). In each data space (ACT, FEA, and PRD), the image vectors are plotted into a 2D space as 2D points through t-SNE projection. Users select these points in one space and meanwhile, the images are highlighted in other spaces. By comparing their distributions, users are hinted for the model behaviors. For example, a close group of images in ACT means that the images have similar actual labels of attributes. But their distributions in PRD space may be far away indicating that the model made wrong prediction. Similarly, departing images in FEA space shows that the neural network finds different high-level features in these images. Then other views provide tools for users to further study these findings.

\begin{figure}[t]\centering
 \includegraphics[trim={0 0.5cm 0 0},clip,width=0.7\columnwidth]{images/AttributeSet.png}
    \caption{An attribute set view in the attribute panel showing the numbers of images with different attribute combinations. } 
    \label{fig:attributepanel} 
\end{figure}

\subsection{Image Exploration from Attributes}
An alternative exploration path is to study the images from their attributes. First, users can interactively select any  combinations among all attributes in the attribute panel. Then an attribute set view shows the model performance of the images with these attributes in Fig. \ref{fig:attributepanel}, where "Many rings", "Ring" and "Strong scattering" three attributes are selected as an example. The bottom row shows there are 34 images that all the three selected attributes are correctly classified (by the dark dots). The top row indicates all the three attributes are not correctly classified in 5 images. Users can click any row so that all the images in the case are selected as one group for further study.

%\begin{figure}[t]\centering
% \includegraphics[width=\columnwidth]{latex/Images/Matrix.png}
%    \caption{\it A matrix view showing a pair-wise coexistence correlation. }\vspace{-5pt} 
 %   \label{fig:matrix} 
%\end{figure}

%Users can further discover image instances based on co-existence cues. As shown in Fig. \ref{fig:matrix}, the top right half of the matrix view shows the correlation of any pair of attributes in ACT and the low left half of the matrix view shows the correlation in PRD. The correlation is based on the model performance over the images having both attributes. Therefore, for example, a large value in PRD indicates the prediction of such images are highly related. Users can click on any cell to select these images as a study group.

\begin{figure}[t]\centering
 \includegraphics[width=\columnwidth]{images/correlation_matrix_updated.png}
    \caption{ Top: Matrix view of pairwise attribute correlation. The blue triangle represents the correlation of two attributes in \hl{PRD}, while the green triangle shows the correlation in \hl{ACT}. Bottom: Martrix view of conditional entropy in the true-label space.}
    \label{fig:matrix} 
\end{figure}

Users can further discover image instances based on co-existence metrics. We visualize these metrics in interactive color enhanced matrices. For both Pearson correlation and mutual information, since changing the order of two attributes will not affect the dependence result, the generated matrix is symmetrical. To save space, we use  half of a matrix to visualize one relationship of two attributes, as shown in the top of Fig.\ref{fig:matrix} where the green and blue triangles form a full matrix. The blue triangle represents the correlation of two attributes in ACT, while the green triangle shows the correlation in PRD. In addition, the values in the diagonal cells are computed with one attribute from ACT and the other from PRD and colored in orange. A high value cell in the matrix indicates high correlation. Users can identify interested pairs of attributes in one triangle, while the same pairs in the other triangle are also highlighted. This design helps users evaluate the model performance by comparing the relationship of the two attributes in two spaces.   

For conditional entropy, the order of the two attributes matters. A full matrix is used for the attributes in either ACT or PRD. The horizontal attributes are conditional attributes  $ \mathbf{Y}$, and the vertical ones are the uncertain attributes $ \mathbf{X}$. We show the matrix for ACT space in the bottom of Fig.\ref{fig:matrix}. For example, zero value cells of the matrix indicate the two attributes are either simultaneously existing (e.g., high orders and many rings) or are mutually excluded (e.g., circular beamstop and linear beamstop). 

\begin{figure}[t]\centering
 \includegraphics[trim={0 0 1cm 0},clip,width=\columnwidth]{images/coexistencetable.png}
    \caption{ A co-existence table view of multiple attributes. It shows the number of images that contain this attribute combination in the true-label space (Number), and the number of correctly predicted images (CorNum).
    }\vspace{-5pt} 
    \label{fig:coexistencetable} \end{figure}

In addition, Fig. \ref{fig:coexistencetable} is the table view of multi-attributes. Here users can choose different number of attributes and three attributes are shown in this figure. The top three attributes can be ranked (with user interaction) by the total number of images with them or the number of correctly predicted images. Users can select any group of the images for further study.


\begin{figure}[t]\centering
 \includegraphics[width=\columnwidth]{images/parallel_new.png}
    \caption{ Two parallel coordinates plots showing attribute measures of model performance with various metrics. }
    \label{fig:PCP} 
\end{figure}

\subsection{Image Group Exploration and Comparison}
While the groups of images are selected, they can be drilled down for the characteristic measures as shown in Fig. \ref{fig:PCP}, where two parallel coordinates plots (PCP) are used to show the measures of each attribute inside one group. On the left, the attributes exist in most images are shown on the top. Users can hover over each attribute to highlight the polyline, while the corresponding images are highlighted in the embedded space views as well. 

The selection of images can also be visualized in a gallery with thumbnail views, as shown in Fig. \ref{fig_CaseRings}. Here, the images are grouped by the number of attributes they include (in ACT or PRD). It is easy for users to identify outliers which may be mis-labelled of attributes.  

Moreover, these images can be displayed in a cluster view as shown in Fig. \ref{fig_interface}(F1-F2). Here the purpose is to further show the relative distribution of the group images. For example, Fig. \ref{fig_interface}(F1) shows two \textit{spatial clusters} generated by applying the K-means algorithm to the blue image points in PRD space in Fig. \ref{fig_interface}(E). This clustered view provides a clearer depiction and easier interaction of the images, comparing with a naive ``zoom-in'' view of these points from Fig. \ref{fig_interface}(E) which is not satisfactory from our experiment with domain scientists. Users can control the number of clusters. Moreover, users can cluster the same selection of images according to the different latent spaces in  Fig. \ref{fig_interface}(F1 and F2).  For example, in contrast with the clusters in PRD space in Fig. \ref{fig_interface}(F1), the same selection of images highlighted by the blue image points were dragged into Fig. \ref{fig_interface}(F2) where shows the two clusters in FEA space and matches with the points distribution in Fig. \ref{fig_interface}(D). Therefore, the group panel can be used for effective comparison.

In addition, an \textit{attribute flower} visualization (Fig. \ref{fig_flower}) is designed (based on Astor charts) to show each attribute as a ``petal''. Each petal is filled in the corresponding color of one selected attribute if the image has this attribute in its ACT vector. The petal has a black border if this attribute does not exist in the ACT vector but appears in its PRD vector. The missing petals simply indicate true negative prediction. Therefore, FN, FP, TP and TN attributes can be easily discerned for each image and for comparison.


\begin{figure}[t] \centering
 \includegraphics[width=0.8\columnwidth]{images/flower2.png}
   \caption{ The attribute flower visualization of images, where each petal represents one attribute. A blank petal indicates FN, a solid petal indicates TP, a missing petal indicates TN, while a solid petal with a black border means FP. }\vspace{-5pt}
   \label{fig_flower} 
\end{figure}

==> sections_version_old/evaluation.tex <==
\section{Evaluation}

\subsection{Interview with Domain Scientists}

We conducted an interview with two domain scientists (working in physical and material sciences) who have some experiences on applying deep learning methods on x-ray datasets. They were given a thorough introduction to the system and its functions. Then, they practiced freely with the system for the investigation of the x-ray scattering data and performed the following study.  These scientists also contributed to the case studies.

\subsubsection{A Usage Scenario:}
Domain experts found two groups with images show big ``ring'' and small ``ring'' on FEA space. In the semantic prediction space and actual label space, these two groups are supposed to indicate the same thing. However, they are separated in the FEA space, which means the neural network takes the scale of the attribute ``ring'' into account \st{quite a lot} \hl{significantly}. This is an interesting point found by the domain expert. It means that in the FEA space, the clusters are formed by the data points visually close to each other rather than semantically. \st{The function of the fully connected layers then have to play the role to cluster the images spreading in more wide area in the FEA space that are semantically share the same attributes.} \hl{ Thus, the function of the fully connected layers have to play the role to collect the visual features which are the same semantically from a more widely distributed area in the FEA space for the classification task.} Since ResNet50 contains only a single fully connected layer to do this work, the domain experts expected that more fully connected layers may be added in the end of the classification phase.   
\begin{table*}[t]				
\caption{QUIS questions and ratings }			\centering				
{\makebox{\resizebox{0.7\textwidth}{!}{				
\begin{tabular}{l|c|c} \hline%\noalign{\smallskip}		
\hspace{30ex} Questions & Means & Standard \\	
 &  &  Deviation\\				\hline%\noalign{\smallskip}				
\textit{Part I: Visual Tools Questions: 0(poor) - 9(excellent)} &\\
\rowcolor{Gainsboro!60}
\textit{Coordinated Visualization with Embedded Spaces} & &\\
Embedded views for showing image groups and outliers. &8.45 &0.52 \\			
Zooming and panning operations.&8.91 &0.30 \\				
Multiple spaces comparison and drill down study. &8.82 &0.40\\
Image item transparency showing errors. &8.27 &0.79 \\			
Image item labeling. &8.36 &0.67\\

\rowcolor{Gainsboro!60}
\textit{Image Group Selection}& &\\
Free selection on embedded spaces. &8.91 &0.30 \\	
Image group management. &8.64 &0.50 \\	
Image group coloring function.&8.82 &0.40 \\	


\rowcolor{Gainsboro!60}
\textit{Image Group Visualization}& &\\
Group panel drag and drop.  &8.73 &0.64 \\
Group measures with PCP. &8.27 &1.27 \\
Group thumbnail gallery overview. &8.63 &0.50 \\
Group spatial clustering. &8.73 &0.47 \\
Image attribute flower view. &8.73 &0.64 \\


\rowcolor{Gainsboro!60}
\textit{Attribute Co-existence Visualization}& &\\
Attribute list with interaction.  &8.64 &0.50 \\
Attribute set view and group selection. &8.36 &0.57 \\
Attribute co-existence table view.  &8.63 &0.57 \\

\rowcolor{Gainsboro!60}
\textit{Detail View Image Visualization}& &\\
Image visual comparison. &8.64 &0.67 \\
Image ACT and PRD value comparison. &8.45 &0.52 \\


\hline%\noalign{\smallskip}				

\textit{PartII. Visual system rating} &\\
\rowcolor{Gainsboro!60}
\textit{Interface} & &\\	
Reading labels and icons on screen. 0(very hard) - 9(very easy)&8.10 &1.04\\				
Highlighting selected focuses in study. 0(not at all) - 9(very much)&8.27 &0.65\\	
Organizing information on the interface. 0(confusing) - 9(very clear)&8.45 &0.69\\				
Sequential operations on the interface. 0(confusing) - 9(very clear)&8.18 &0.98\\			
Interaction on visual tools. 0(very hard) - 9(very easy)&8.23 &0.79\\

\rowcolor{Gainsboro!60}
\textit{learning} & &\\
Learning to operate the system. 0(difficult) - 9(easy)&7.18 &1.17\\
Performing tasks is straightforward. 0(never) - 9(always)&8.09 &0.83\\

\rowcolor{Gainsboro!60}
\textit{System} & &\\				
System response with good speed. 0(very slow) - 9(fast enough)&8.36 &0.81\\				
Designed for all levels of users. 0(never) - 9(always)&7.82&1.32\\		
System reliability. 0(unreliable) - 9(very reliable)&8.18 &0.75\\		\hline%\noalign{\smallskip}				
\end{tabular}				
}}} \vspace{-5pt}
\label{table:QUIS}				
\end{table*}		
\subsubsection{Feedback on Usability} 
Based on the experience with the usage scenario, the domain scientists provided feedback on the system usability in physical and material research. Next is the summary of the feedback on good points and limitation.

\noindent \textbf{Good points:}
\begin{itemize}
\item \textit{About system interface:} This interface allows users to explore the training data and the trained model side-by-side. The tool is very easy to explore and identify the issue of the model.

\item \textit{About interlinked embedded views:} The linking of data between embedded views is extremely important and well executed. This allows users to follow a chain of logic from one representation to another to study model performance.

\item \textit{About outliers and hypotheses:} The system both allows users to explore and search for outliers, as well as to test hypotheses by grouping data and performing analytic tests. This kind of interaction is extremely useful for being able to then refine the training model. 

\item \textit{About model behavior:} Perhaps more importantly, this tool allowed users to identify limitations and biases in the training data itself. Thus, this tool is a useful guide towards improving training datasets.

\end{itemize}


\noindent \textbf{Limitation and suggestion:}
\begin{itemize}
\item \textit{About network layers:} Only the feature space after all convolutional layers are used, it would be good to further show the study of the feature maps from other layers in the deep network.

\item \textit{About embedded space control:} For embedded spaces, it is very useful to see how data is organized. However, because the true spaces are high dimensional, it would be nice to have more control over how one is viewing the ``true space'', such as using alternate layout modes, ability to rotate view, etc.

\item \textit{About group study:} For group study panel, it requires some training to know how to use them and interpret the information. Perhaps some additional feedback to users could make these tools more immediately understandable.
\end{itemize}

\subsection{Evaluation for Visual Interactions}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\noindent \textbf{Participants:} Eleven graduate students who are computer science majors (4 females, 7 males) participated in the evaluation of the visual system. All the participants had  knowledge of visualization and interface design and experience in web-based visualization tools. Six of them have experiences of deep learning models and tools. 

\noindent \textbf{Procedures:} An instructor first introduced the x-ray scattering images and structural attributes, and then the visualization and interaction functions to each participant. They were guided to freely explore the system with image data for about 10 minutes. Then, they completed the tasks: (a) find outliers in an image group; (b) discover the model behavior of attributes in the image groups. Afterwards, they provided the evaluation by filling a QUIS (Questionnaire for User Interaction Satisfaction) form which is widely used in human computer interface evaluation \cite{Chin1988}. Finally, they gave comment and suggestions for the system.

\noindent \textbf{QUIS evaluations:} 
Table \ref{table:QUIS} shows the questions and ratings in two parts about: 1) The visualization design and functions, and 2) The system performance. The mean and standard errors of the user ratings are displayed as well.

The average score of the visualization and interaction functions are very good above 8.0, which indicates the users were satisfied overall. For example, the interactive operations on the embedded spaces like ``Zooming and Panning'' and ``Free selection'' received excellent rating with an average of about 8.91. ``Multiple spaces comparison and drill down study'' also got high average score 8.82. It indicated that the interaction to exploring data in the embedded spaces was well implemented.

The ratings of the visual system are also very good. The Web-based system performance with fast response impressed the users. They also felt the system layout and organization was easy to follow. The average rating scores for ``Learning to operate the system'' and ``Designed for all levels of users'' were good but relatively lower at 7.18 and 7.82. The standard deviations of these two were also high at 1.17 and 1.32. This is reasonable as the users need to understand the deep learning model performance over the scientific images. In future work, we will add more labels and guidance in the system to shorten the learning curve. 

The users' comments also identified system limitations to be further addressed. For example, visual clutters appear when the image labels of a large group of selected images are shown in the embedded spaces. Here, a smart labeling algorithm is needed. In addition, the selected groups is fixed and more flexibility may be added to insert and delete specific images to/from a group. Moreover, the color selection for different attributes should be adjustable by user-definition. We will further improve the system according to these suggestions.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\subsection{Discussion}
Visual interaction tools are helpful for trainers and users of deep learning models \hl{in scientific domain}. For the x-ray scientific images, extra challenge arises from the complex structures which co-exist, overlap, and often have drastic variations in their shapes and formats. First, the direct use of existing scientific categories of attributes in deep learning models may not be very effective. For example, ``ring'' may be further divided into different types as found in the case study. Second, the training data based on the labeling of domain scientists often suffers from more mis-labels and errors than natural images. An effective labeling tool may be developed to improve the accuracy and effectiveness of labeling process itself. 

\hl{Besides, the scalability of this system also allows to apply it on other natural image datasets and the corresponding models. The data labels can be updated from a text file by clicking the button “Load Feature Names” in the top of the navigation bar. Meanwhile, the extracted and preprocessed three vectors will be loaded correspondingly to the system from the database. This makes it flexible to do analysis even on the model classification of single attribute dataset like Cifar10. In that case, the roles and their detail contribution from the rest of all non-target attributes of an image can be revealed. It helps to diagnose the reason for the wrongly predicted image.}

==> sections_version_old/introduction.tex <==
\firstsection{Introduction}
\maketitle

X-ray scattering helps scientists discover molecular and nano level physical structures of materials such as nano-particles, protein, lithographic gratings, polymer films, and so on. The technique is widely used in biomedical, material, and physical applications by analyzing structural patterns in the x-ray scattering images \cite{Yager2014}. X-ray equipment can generate up to 1 million images per day which impose heavy burden in post image analysis. A variety of image analysis methods are applied to x-ray scattering data. Recently, deep learning models are employed in classifying and annotating multiple image attributes from experimental or synthetic images, which were shown to outperform previously published methods \cite{Wang2017,Guan2018}. As most deep learning paradigms, these methods are not easily understood by material, physical, and biomedical scientists. The lack of proper explanations and absence of control of the decisions would make the models less trustworthy. While considerable effort has been made to make deep learning interpretable and controllable by humans \cite{Choo2018}, the existing techniques are not specifically designed for the scientific image classification models of x-ray scattering images, which requires extra consideration in finding: 
\begin{itemize}
    \item How the learning models perform for a diverse set of overlapped image attributes with high variation?
    \item How the co-existence of attributes in x-ray images may affect the classification results? 
\end{itemize}
Unfortunately, few existing visualization tools \cite{Choo2018} are devoted to visually analyzing the learned results of multiple attributes, objects, or segments with these models.

In response, we develop a visual analysis system for users to interactively study the model predictions with respect to the multiple structural attributes of x-ray scattering images. The system has several features:
\begin{itemize}
    \item Image instances are projected with t-SNE and visualized in three vector spaces: actual labeling space from domain scientists, feature space extracted by a residual network, and prediction space of the model output. Users can explore the instances in these spaces interchangeably for visual comparison of different groups, outlier detection, and drill-down study of images.
    \item Users can select any image group and then observe their visual features and study the attribute detection performance. In particular, the distributions of these images in different spaces are easily discovered by user controlled spatial clustering in the embedded spaces.  
    \item An attribute-flower visualization is designed to represent an image to manifest the attribute recognition results. Compared with the ground truth labels, it depicts false positive (FP), false negative (FN), true negative (TN), and true positive (TP) predictions of multiple attributes.
    \item The learning outcome of the images with different groups of co-existed attributes are visualized, which provides visual cues of model performance with respect to attributes relationships.
    \item The visual interface integrates multiple coordinated views and includes easy user interactions that facilitate iterative exploration and comparison.
\end{itemize}
The system alleviates domain scientists' efforts in understanding the performance of deep learning models for x-scattering images. They can identify outlier images, find spurious data clusters, understand impacts of multiple attributes, and from this either improving the training data or the learned model. Several case studies show the utility and effectiveness of the system. Domain scientists provide positive feedback about the usefulness of this visual interaction tool.

==> sections_version_old/network.tex <==
\section{Neural Network Learning of Multiple Structural Attributes}
\subsection{X-Ray Scattering Images}

\begin{figure}[t]\centering
 \includegraphics[width=\columnwidth]{images/Images162_67_ResNet.png}
    \caption{ X-scattering images and ResNet model. (Left) Two images including ``Halo'' and ``Ring'' attributes. (Right) ResNet50 architecture \cite{He2016}. }
    \label{fig:resnet} 
\end{figure}

Automatic attribute recognition in x-ray scanned image data is a challenging problem due to the high variation in the same classes. The same structural attributes (patterns) can be of great variety in their appearances. On the other hand, a diverse set of characteristic attributes, from the type of measurement, e.g. ``small-angle x-ray scattering (SAXS)'' or ``wide-angle x-ray scattering (WAXS)'', to instrumental information, e.g. ``linear beam stop'' or ``beam off image'', to appearance-based scattering features, e.g., ``halo'' or ``ring', may co-occur and overlap in the scattering images. As shown in Fig. \ref{fig:resnet}, two images both include ``Halo'' and ``Ring'' attributes and other attributes. Scientists want to seek help from deep learning models to identify these features in given images. In our prototype, we utilize an open x-ray scattering dataset \cite{Yager2017} and the ResNet model in \cite{Wang2017} for our design of visual analytics techniques.

We retrieved about 1,000 x-ray scattering images from the dataset \cite{Yager2017}. They include different types of images including semiconductors, nano-particles, polymer, lithographic gratings, and so on. The attributes in these images are either labelled by domain experts or synthetically generated by a simulation algorithm \cite{Wang2017}. Each image thus has an actual attribute vector (\textbf{ACT vector}) consisting of 17 Boolean (0 or 1) values to show if the image has one of the 17 attributes. 

\subsection{ResNet Deep Learning Model and Data Spaces}
A 50-layer Residual Network (ResNet) proposed in \cite{He2016} was trained for the 17 attributes by more than 100,000 x-ray images. Fig. \ref{fig:resnet} shows the abstract architecture of this model. It has the first 50 hidden convolution layers for the feature extraction. A feature vector (\textbf{FEA vector}) with 2048 dimensions was learned by the model for each image. Then, after average pooling, a fully connected layer is used for predicting existing structural attributes. The fully connected layers generated final output of a prediction vector (\textbf{PRD vector}) for the 17 attributes. The deep learning model reported a mean average precision (mAP) about 77\% \cite{Wang2017}. 

From the model, the x-ray images are represented by vectors in three different spaces (i.e., ACT, FEA, and PRD). The ACT vector has 17 dimensions with each being the Boolean label corresponding to one attribute. The PRD vector with the same size 17 is obtained from the output of the trained ResNet model with fully connected layers for classification \cite{Wang2017}. Each PRD element is the prediction probability (0.0 to 1.0) for each attribute with a cut-off value of 0.5 for final decision. The FEA vector with the size of 2048 dimensions contains the activation values of the last feature extraction layer in ResNet \cite{He2016}. The characteristics of an image are supposed to be extracted and representative by its FEA vector, though it is not directly interpretive. Comparing the images in these spaces can reflect the performance of the ResNet for x-ray scattering images.
 
\subsection{Model Performance Measures}
Model performance metrics help users understand and study the model output and performance. They will play the role as visual cues for effective interactive exploration.

For a set of x-ray scattering images, the prediction output of the learning model generates the values of false positive (FP), true positive (TP), false negative (FN), and true negative (TN) for each specific structural attribute. For example, FP($\alpha$) values of one attribute ($\alpha$) shows the number of images who does not include $\alpha$ in ACT but shows positive prediction in PRE. Based on the four values, four metrics are used to evaluate model performance of each attribute $\alpha$: 
\begin{eqnarray}
Accuracy(\alpha) = \frac{TP(\alpha) + TN(\alpha)}{TP(\alpha) + TN(\alpha) + FP(\alpha) + FN(\alpha)}, 
\\
Precision(\alpha) = \frac{TP(\alpha)}{TP(\alpha)+FP(\alpha)}, 
\\
Recall(\alpha) = \frac{TP(\alpha)}{TP(\alpha)+FN(\alpha)}, 
\\
F1(\alpha) = 2 \times \frac{Precision(\alpha)\times Recall(\alpha)}{Precision(\alpha)+ Recall(\alpha)}.
\label{eqn:individualmetrics}
\end{eqnarray}

The accuracy is affected by the sum of TP and TN. The precision (recall) suffers only when FN (FP) is large. F1 score instead makes both FN and FP from precision and recall in balance. 

Considering multiple attributes appearing on one image, a statistic metric of average precision (AP) (or mean AP) can be used. For evaluating object detection (such as in ImageNet), it is often defined by an AUC (area under curve) method which in general computes the area under the precision-recall curve \cite{Su2015}. While it gives a quantitative evaluation for the model, it only gives a global measure for the dataset and cannot be used for drill-down study.


\subsection{Co-existence Relationship of Attributes}  \label{sec:coexistence}

Having multiple attributes on the same images is a unique feature of x-ray scattering images. It is of interest and importance for scientists to discover the impact of attribute relations for model performance. 

\subsubsection{Pairwise co-existence} 
For two attributes, we employ the measures of Pearson correlation, mutual information, and conditional entropy.

Pearson correlation coefficient is a measure of linear dependence of two variables. The range of value is from -1 to +1, and its geometric interpretation is similar to the dot product, which also measures the cosine angle of two linear dependent variables. As in Eqn.\ref{eqn:correlation}, when $r_{\scaleto{\mathbf{X}\mathbf{Y}}{3pt}}$ is zero, variable $x$ and $y$ have no linear relationship, while 1 (-1)  means perfect positive (negative) linear dependence.

\begin{equation}
    \label{eqn:correlation}
    r_{\scaleto{\mathbf{X}\mathbf{Y}}{3pt}} = \frac{{}\sum_{i=1}^{n} (x_i - \overline{x})(y_i - \overline{y})}
{\sqrt{\sum_{i=1}^{n} (x_i - \overline{x})^2(y_i - \overline{y})^2}}
\end{equation}

Mutual information also quantifies the mutual dependence of two random variables, and it is not limited in the relationship of the linear dependence. It measures the reduction of uncertainty of one attribute due to the knowledge of another attribute: 
\begin{equation}
\label{eqn:mutual_information}
I(\mathbf{X}; \mathbf{Y}) = \sum_{x\in \mathbf{X}}\sum_{y\in \mathbf{Y}} p(x, y)\log \frac{p(x, y)}{p(x)p(y)}.
\end{equation}

Conditional entropy measures the uncertainty of one attribute, under the conditional state of another attribute. It can reflect weighted average uncertainty of this unknown attribute, given all possible states of known attributes:

\begin{equation}
\label{eqn:conditional_entropy}
H(\mathbf{X} | \mathbf{Y}) = - \sum_{x\in \mathbf{X}}\sum_{y\in \mathbf{Y}} p(x,y)\log \frac{ p(x,y)}{ p(x)}.
\end{equation}

Here, in both Eqn.\ref{eqn:mutual_information} and Eqn.\ref{eqn:conditional_entropy}, $ \mathbf{X}$ and  $\mathbf{Y}$ both have two possible values 0, and 1, referring to these two attributes existing or not in one image. Based on them, $p(x)$ and $p(y)$ can be computed as marginal probabilities of the two attributes, and $p(x,y)$ as their joint probability, occurring in a group of images. 

%%%%%%%%%%%%%%%%%%%%
% For two attributes, we employ the measures of mutual information, correlation, and conditional entropy. 

% Mutual information quantifies the mutual dependence of two random variables. In our case, it measures the reduction of uncertainty of one attribute due to the knowledge of another attribute. 
% \begin{equation}
% \label{eqn:mutual_information}
% I(\mathbf{X}; \mathbf{Y}) = \sum_{x\in \mathbf{X}}\sum_{y\in \mathbf{Y}} p(x, y)\log \frac{p(x, y)}{p(x)p(y)}.
% \end{equation}
% Here $x\in \mathbf{X}$ has four cases referring to the model performance metrics of TP(X), TN(X), FP(X) and FN(X). ?? $p(x,y)$ is the joint probability of these attributes occurring together in an image. 

% The joint entropy is computed as
% \begin{equation}
% \label{eqn:entropy}
% H(\mathbf{X}, \mathbf{Y}) = -\sum_{x\in \mathbf{X}}\sum_{y\in \mathbf{Y}} p(x,y)\log p(x,y),
% \end{equation}
% which provides a measure of uncertainty (in the context of information theory) associated with the two attributes. It provides information about the variation, or diversity, of the images containing the two attributes.

% Pearson correlation: XXX
\subsubsection{Multivariate co-existence}

A variety of metrics \cite{Timme2014} measure  multivariate relationship with more than two attributes. They can be visualized through multi-dimensional visualizations. However, based on our experiment, these multivariate measures are hard to be understood by domain users as visual cues of the x-ray learning model results. Therefore, we enumerate all real combinations of multiple attributes within the image dataset, for example, any pair of two attributes, and 3-tuples of three attributes, etc. For each combination, the prediction accuracy are represented by finding whether all the involved attributes are correctly detected. By visualizing this information, users can find which set of co-existed attributes are interesting for further study. Note that a large number of attributes (more than 8) do not appear together in one image so that this approach is valid.


==> sections_version_old/relatedwork.tex <==
\section{Related Work}
It is of great importance to analyze x-ray scattering images by recognizing structural attributes such as ring, halo, diffuse scattering, and so on. \cite{Kiapour2014}. Recently, deep learning models are employed for the x-scattering data \cite{Sullivan2019, Park2017,Liu2019}. Wang et al. \cite{Wang2017} apply Convolutional Neural Networks (CNN) over both experimental and synthetic images to detect important attributes. Guan et al. \cite{Guan2018} further develop a DVFB-CNN model which combines Fourier-Bessel transform (FBT) within CNN model. 

Choo et al. \cite{Choo2018} categorize explainable deep learning into three major directions: model understanding, model debugging, and model refinement. Computational approaches discover importance scores of the input features contributing to the prediction results. Perturbation methods \cite{Alvarez-Melis2017}, saliency based methods \cite{Selvaraju2016}, LIME \cite{Ribeiro2016}, and influence functions \cite{Koh2017} are proposed for the purposes. Interactive visualization tools are developed in providing in-depth understanding of how deep learning models work. Tools such as Tensorflow \cite{Wongsuphasawat2018} Playground, Tensor Board, and ConvNetJS \cite{ConvNetJS} allow users to visualize and interact with the activation maps and network structures, together with line graphs and histograms of characteristic statistics. DeepVis \cite{Yosinski2015} shows that optimizing synthetic images with better natural image priors produces more recognizable visualizations. CNNVis \cite{Liu2017} system helps designers in their understanding and diagnosis of CNNs by exploring the learned representations in the graph layout of the neural networks. ActiVis \cite{Kahng2018} integrates embedding view with multiple coordinates views for visual model exploration. Embedding Projector \cite{EmbeddingProjector} visualizes input images in a 2D or 3D embedding space (by PCA or t-SNE), to reveal the relationship among these instances. For studying the training process, Deep View \cite{Zhong2017} presents a level-of-detail framework that measures the evolution of the deep neural network both on a local and on a global scale. Recently, visualization tools \cite{Wang2018a,Liu2018,Kahng2019} have been developed for studying deep generative models (e.g. GAN) working on benchmark natural images. These methods have not been specifically designed for x-ray scattering images. 



Our approach allows users to analyze the results of physical attributes recognition in special scientific image data, where multi-attributes may have inherent correlations and co-exist in one x-ray image. And these relationship among attributes may play important role and affect the performance of the trained model predictions for each image. Therefore, it is different from those existing tools to analysis the disjoint multi-attributes classification in the existing works\cite{Pezzotti2018,Rauber2017,Rauber2016,EmbeddingProjector,Maaten2008,Zhong2017}. 
 Though it may be similar to multi-objects co-exist in a big natural image, the scientific attributes have large structural variations (e.g., rings can be very large circular structure and can also be very small and indiscernible by eyes)\cite{Zhao2019}. There is a dire need of effective visualization tools to discover the relationship among the scientific structural objects on scientific images and the performance of deep learning models\cite{Choo2018}. 
 Our system is different from most existing methods, in which image, audio and natural language datasets are projected and visualized by linking the final decision with the origin images/text data elements, but not the individual attributes (objects). The visualization focusing on multiple structures on the images may in the future be extended to deep learning models for multiple object detection and segmentation, such as (fast-, faster-) R-CNN \cite{Zhao2019}, YOLO \cite{Redmon2017}, and SegNet \cite{Badrinarayanan2017}. 

This paper presents techniques on model understanding, according to the categories in Choo et al. \cite{Choo2018}, with the trained ResNet model of x-ray scattering images. \st{Model debugging and refinement tasks for improving the training process will be our future work}.


==> test.tex <==
\firstsection{Introduction}

\maketitle
\textbf{Do not Read Introduction, JUNK Information right now copy pasted}\\

\textit{Direct Volume Rendering of Photographic Volumes Using Multi-Dimensional Color-Based Transfer Functions}
Increasingly, photographic volumes are becoming a viable
and important means to represent anatomical and pathological information. Not only is the ability to acquire and
compose data in this manner progressing but, the advantages that they hold over traditional data acquisition techniques(i.e. CT, MRI) have been further realized. A lack of
adequate resolution provided the impetus for the Whole Frog
Project at Lawrence Berkeley National Laboratory to use
photographs of cryosections to create a volume dataset of an
entire frog26. Other examples of cryosection imaging can be
found at UCLA’s Laboratory for Neurological Imaging and the Armed Forces Institute of Pathology’s Visible Embryo
Project. The most comprehensive examples of data acquisition using photographic tomographic imaging are the Visible
Female and Visible Male datasets produced by the National
Library of Medicine36 these volumes in a fashion that yields information previously
not obtainable from "traditional" clinical data sets or volume
rendering methods. Recently, color-based transfer functions
were designed that would facilitate the generation of compelling volume renderings of these datasets. These transfer
functions were based solely on the three channel color space
(RGB or CIE Luv) of the photographic datasets. Both
color distance gradient magnitudes and color distance gradient dot products were used to map the voxel’s color information to an opacity value. When coupled with volume
illustration techniques
, where a physics-based illumination
model is used in conjunction with non-photorealistic rendering (NPR) methods, there is the potential for a powerful
technique in which to convey the structure of a photographic
volume model.
Though these transfer functions succeed in extracting
many boundaries within the volume, the opacity of a voxel
was largely based on the gradient magnitude at that voxel.
For a more exact determination of a boundary region, another measure is needed. It has been demonstrated that volumes of scalar data suggest their own appropriate transfer
function when boundaries between different materials are
the primary regions of interest17. Furthermore, these transfer functions can be determined by the relationship between
the original data value and the first and second directional
derivatives along the gradient direction. This notion applies
to photographic volumes where the data values are the color
components and a significant change in these color components denotes a boundary of some sort. We build upon the
utility of the color-based transfer functions and the volume
illustration techniques by applying them simultaneously and
adding a component based on the second directional derivative, namely the zero-crossing within this derivative. By adding this component, we have strengthened our method
for determining boundaries within a photographic volume
and subsequently, our renderings from photographic volumes.\\

\textit{Multidimensional Transfer Functions for Interactive Volume Rendering}
DIRECT volume rendering has proven to be an effective
and flexible visualization method for three-dimensional
(3D) scalar fields. Transfer functions are fundamental
to direct volume rendering because their role is essentially
to make the data visible: By assigning optical properties like
color and opacity to the voxel data, the volume can be
rendered with traditional computer graphics methods.
Good transfer functions reveal the important structures in
the data without obscuring them with unimportant regions.
To date, transfer functions have generally been limited to
one-dimensional (1D) domains, meaning that the 1D space
of scalar data value has been the only variable to which
opacity and color are assigned. One aspect of direct volume
rendering which has received little attention is the use of
multidimensional transfer functions.
Often, there are features of interest in volume data that
are difficult to extract and visualize with 1D transfer
functions. Many medical data sets created from CT or
MRI scans contain a complex combination of boundaries
between multiple materials. This situation is problematic
for 1D transfer functions because of the potential for
overlap between the data value intervals spanned by the
different boundaries. When one data value is associated
with multiple boundaries, a 1D transfer function is unable
to render them in isolation. Another benefit of higher
dimensional transfer functions is their ability to portray
subtle variations in properties of a single boundary, such as
its thickness. When working with multivariate data, a
similar difficulty arises with features that can be identified
only by their unique combination of multiple data values. A
1D transfer function is simply not capable of capturing this
relationship.
Unfortunately, using multidimensional transfer functions
in volume rendering is complicated. Even when the
transfer function is only 1D, finding an appropriate transfer
function is generally accomplished by trial and error. This is
one of the main challenges in making direct volume
rendering an effective visualization tool. Adding dimensions
to the transfer function domain only compounds the
problem. While this is an ongoing research area, many of
the proposed methods for transfer function generation and
manipulation are not easily extended to higher dimensional
transfer functions. In addition, fast volume rendering
algorithms that assume the transfer function can be
implemented as a linear lookup table (LUT) can be difficult
to adapt to multidimensional transfer functions due to the
linear interpolation imposed on such LUTs.
A previous paper [19] demonstrated the importance and
power of multidimensional transfer functions. This paper
extends that work with a more detailed exposition of the
multidimensional transfer function concept, a generalization
of multidimensional transfer functions for both scalar
and multivariate data, as well as a novel technique for the
interactive generation of volumetric shadows. To resolve
the potential complexities in a user interface for multidimensional
transfer functions, we introduce a set of direct
manipulation widgets which make finding and experimenting
with transfer functions an intuitive, efficient, and
informative process. In order to make this process genuinely
interactive, we exploit the fast rendering capabilities.\\

\textit{Effective Transfer Function for Interactive
Visualization and Multivariate Volume Data}
Volume rendering has been widely employed in
visualization of volumetric data, especially for medical
application. Rather than experienced mental reconstruction of
3D structures of objects slice by slice, volume rendering can
display the details of the volume data set intuitively using
interactive graphics and imaging methods. Transfer function
plays an essential part in volume rendering since its capability
of mapping optical properties like color and opacity to voxel
data to reveal occluded objects. The transfer function affects
the final image to a great extent, and moreover is directly
related with the user's understanding of the volume data sets
[1].
The easiest way to design the transfer function is the trialand-
error method. However, volume data sets often require a
lot of trials and the ideal transfer function may be missed
because of the lacking of guiding information. To overcome
the difficulty of the design of trial-and-error transfer function,
recent research has focused on automatic and semiautomatic
techniques for transfer function design. Earlier transfer
functions are limited to one dimensional (1D) domains. Bajaj et
al. [2] introduced a data-centric method that generates the
contour spectrum to help the user determine those scalar values
which correspond to unique isosurfaces. Fujishiro et al. [3],
aimed at finding important isosurfaces by investigating their
behavior while changing the isovalue. At certain values,
surfaces split or merge. Such surfaces were then emphasized in
the visualization. He et al. [4] presented an image-centric type
of automation which optimizes visualization parameters using
the random search and a genetic algorithm to design the
optimal 1D transfer function. Marks et al. [5] and König and
Gröller [6] proposed design galleries as an interaction with the
user.
Due to the complexity and diversity of volume data,
features of interest in volume data set are difficult to extract
and visualize only with 1D transfer functions. Levoy treats the
transfer function as a two dimensional function, where voxel
intensity and the corresponding gradient value are used to
classify the medical data [7]. Other approaches further take
curvature into account to help distinguish between objects
according to their shapes [8]. Tzeng et al. [16] used a highdimensional
learning classifier for the volume visualization.
Shape-based [17], size-based [18] and topology-based [3]
transfer functions have been proposed that classify the local
structure of volume data.
In most cases, boundaries carry the important information
such as the shape and the size of the material, as well as the
spatial relationship with other materials. To display the specific
boundary and to differentiate between boundaries, proper
transfer function design is required. Kindlmann and Durkin [9]
combined the scalar value of data and its first and second
derivatives, and created a 2D histogram in which the
boundaries appear as arches. Kniss et al. [10] used this domain
for their 2D transfer functions. Although the arches enable
some distinction between boundaries, they often overlap
causing selection ambiguities. Šereda et al. [11] went further
and created so called LH space by tracing the boundary profiles
in every voxel to determine the start and end of the arches. It
was shown that in the LH space the boundaries appear as blobs
and are much easier to separate.
Increasing momentum recently is tending to integrate
visualization with interaction to facilitate manipulating and
exploring data for many applications. With the help of
interaction, specifying transfer functions can be made more
intuitive and convenient to better query or manipulation of
specific objects. Piringer and his colleagues describe the use of
brushing interface in the 2D views to specify features of
interest to highlight in linked 3D views [12]. ˇSereda and
Vilanova [11] designed a set of direct manipulation widgets
and revealed boundaries between objects intuitively and
interactively with these widgets.
Multi-dimensional transfer functions could be beneficial in
visualization of multivariate volume data which contains, at
each sample voxel, multiple scalar values. The values represent
different simulated or measured quantities. It is often the case
that a feature of interest in these data sets cannot be properly
classified using any individual variable. Current volume
rendering approaches for visualizing multivariate datasets rely
on designing transfer functions separately for each modality,
and then combine them [13]. Different data values can be
assigned to the different axes of the transfer function. The
composite visualization can simply overlay the classified
modalities or use portions of the different transfer functions, for
instance color from one modality and opacity from another.
Kniss [14] explored the utility of multi-dimensional transfer
functions for the visualization of high resolution multivariate
weather models. Markus Glatter [15] developed a system that
supports efficient visualization of an arbitrary subset, selected
by range-queries, of a large multivariate time-varying dataset.
In this paper, a simplified LH histogram is presented for
transfer function design to interactively visualize the multiboundary
of volume data sets. To reduce the partial volume
effect on the boundary, f-LH histogram is proposed to classify
each side of boundary. Then an effective multi-dimensional
transfer function is designed for visualizing multivariate heart
data.
The reminder of the paper is organized as follows: In
Section 2, the proposed simplified LH histogram and improved
f-LH histogram is described. In Section 3, multi-dimensional
transfer function is designed for multivariate heart data. In
Section 4, experimental results are provided. Finally,
concluding remarks are given in Section 5.\\

\textit{Style Transfer Functions for Illustrative Volume Rendering}

Volume rendering is a well established method for the visualization
of scientific data, such as tomographic scans. Historically,
most volume rendering techniques are based on an
approximation of a realistic physical model. It was noticed,
however, that traditional depictions of the same types of data
– as found in medical textbooks, for example – deliberately
use non-realistic techniques in order to focus the viewer’s
attention to important aspects [ER00,RE01]. Using abstraction,
visual overload is prevented leading to a more effective
visualization. Recent approaches have considered this fact,
leading to an increased interest in illustrative volume visualization.
Approaches for illustrative volume visualization frequently
employ non-photorealistic rendering techniques to
mimic the style of traditional illustrations. They take advantage
of the illustrators’ century-long experience in depicting
complex structures in an easily comprehensible way. Many
of these techniques require tedious tuning of various parameters
to achieve the desired result.We aim to circumvent this
† E-mail: {bruckner|groeller}@cg.tuwien.ac.at
issue by presenting the user with a gallery of styles extracted
from actual illustrations.
For this purpose, we introduce the concept of style transfer
functions. Instead of defining a color transfer function
which is augmented with various parameters for controlling
the non-photorealistic rendering, our approach allows
the user to directly specify styles captured from existing artwork
in the transfer function. Style transfer functions allow
the generation of volumetric illustrations in the style of a
given work of art (see Figure 1).
Contours are an important concept to enhance the stylized
depiction of volume data. We present a simple measure
to calculate the curvature along the viewing direction which
is used to control the thickness of style-based contours. Our
approximation is computationally very efficient since it does
not require explicit reconstruction of second-order partial
derivatives. Using this curvature measure, we also introduce
a new transparency model based on techniques commonly
found in traditional illustrations. Our implementation is capable
of producing high-quality illustrations of volume data
using a wide variety of different styles at interactive frame
rates.

The Visible Human datasets were created as part of a
project to study the potential of using photographic volumes in anatomy research and education. Computed tomography(CT), magnetic resonance imaging (MRI), and plain
film radiographs were used to collect data from both a male
and female subject. The subjects were then frozen and sectioned in 1 mm and 1/3 mm axial intervals for the male
and female subjects, respectively. These sections were subsequently photographed with 35mm and 70mm film and digitized using an electronic camera. The resulting resolution
of the digital images is 2048x1216 and 4096x2700 for the
data generated from the 35mm and 70mm film, respectively.
These datasets represent one of the most complete and extensive anatomical studies ever performed.
With the availability of these high-resolution datasets, an
interesting problem develops of how to effectively render

In this paper, we introduce
%% \section{Introduction} %for journal use above \firstsection{..} instead

\textbf{TF Fundamentals - - - }
Perhaps one of the most important aspects of the TF is the freedom
it provides users in designing visual appearance. The TF further
allows users to interactively alter the visual parameters and their
application to different parts of the object of study. The number of
attributes is increasing, and the usability of available TF tools is
improving. Thus, the TF is increasingly becoming an instrument for
the exploration of scientific content of the data to produce, both scientifically
relevant and aesthetically appealing, high quality images.
The role of the TF as a design and workflow tool was already apparent
in the Transfer Function Bake-Off [PLB01], which analyzed
four approaches in the TF design and highlighted differences in the
workflow of the TF design process.\\

Another trend is the use of a TF as a tool for the expression of user
knowledge of material presence and properties, which transforms
the TF into a source of information that can be used to derive
further attribute data. High level expressions of knowledge codify
the complex relations between data domains and the corresponding
TFs and indeed between different TF segments. A powerful scheme
is to define the TF as material presence components, which follows
the ideas presented by Lindholm et al. [LLL10], where labels
are assigned to TFs with semantics, indicating, for instance, bone,
muscle, fat, etc. Several important contributions to the field rely
on the expression of knowledge encoded in the TF in ways that go
beyond the traditional TF domain. Such approaches have been used,
for instance, in data reduction and multiresolution representations.
\section{Related Work}
\textbf{Do not Read Related Work, JUNK Information right now copy pasted}\\


\textbf{Dimensionality - - - }
Volumetric data is commonly presented as scalar, bi-variate, or multivariate.
Examples of scalar data are medical data from CT scanners
and particle density fields from numerical simulations. Bi-variate
data is also found in medical imaging from dual energy CT scanners
as well as in complex fields, with real and imaginary values, from
numerical simulations in many different domains. There are many
examples of multivariate volumetric data, often from numerical
simulations in fluid dynamics, that create vector or tensor data, but
also from seismic surveys and astrophysical numerical simulations.
Multimodal data is also a common form, in which the data may be
represented on grids with different extent and alignment, such as
Ultrasound B-mode data together with CT data.\\


\textbf{Mutlitdimensional Data - - - }

If the user is to manipulate the TF definition directly, moving beyond
2D TFs immediately poses significant challenges in terms of
user interfaces and cognitive comprehension. Much research and
work on MD TFs is, therefore, related to various forms of automation
and advanced user interfaces, which are covered in Sections
7 and 8. Typical approaches include dimensional reduction, clustering
and grouping, machine learning, and various user interface
approaches such as parallel coordinates or direct slice or volume
view interaction.\\

Another form of MD TFs deals with the classification of color
data, as in the cases of the Visible Human Project, which generated
slice stacks of photographs. The challenge here is to produce a
useful volume rendering that reveals structures within the data, since
color ranges are highly overlapping and ambiguous. Morris and
Ebert [ME02] propose a method to map color data to opacity TFs
to reveal the interior structures of the data. They use boundary
enhancement techniques, which incorporate the first and second
directional derivatives along the gradient direction. The CIEL*u*v*
color space is chosen in their algorithms, and a deeper analysis
is provided in Ebert et al. [EMRY02]. For medical RGB color
data, Takanashi et al. [TLMM02] perform independent component
analysis (ICA) of the RGB-color histogram space. Their assumption
is that moving a clipping plane along the ICA axes allows the user to
discriminate different parts of the data. Muraki et al. [MNKT01] use
a similar ICA-based approach to transfer colors from RGB datasets
to multichannel MRI volumes.\\

\textbf{Aggregated Attributes - - - }
Conceptually, the introduction of additional quantities in the TF
definition makes it possible to discriminate more parts in a dataset.
In practice, however, any added quantity makes it more difficult
to create the TF. Visually, 1D TFs can be represented as a line
or curve, but in the case of 2D TFs, visualizing and modifying
polygons becomes significantly more complex. 3D TFs require
volume rendering of the TF itself, which in turn, requires “meta
transfer functions” for display, making the approach impractical. To
avoid these issues, and going beyond 3D TFs, several papers have
been published suggesting approaches for aggregating attributes
and reducing the complexity of visualizing and designing higherdimensional
TFs.\\


Maciejewski et al. [MWCE09] describe a method for 2D clustering
in a feature space, comprised of value and gradient. The
technique automatically generates a set of TF components that can
be refined or filtered out later in the workflow. The method also
incorporates temporal changes by building a histogram volume from
the 2D feature space, which allows for a more consistent clustering
over time.\\

\textbf{Dimension Reduction - - - }
Dimensionality reduction methods propose simplifying the complexity
of the TF design process by projecting high-dimensional TFs to
a lower-dimensional space. Kniss et al. [KUS05] have presented
an approach for statistically quantitative volume visualization in
which a graph-based technique is used to achieve dimensionality
reduction.\\

\textbf{Color and Texture - - - }
One interesting way of computing a TF is by attempting to apply
realistic looking colors to gray level volume data by either coloring
voxels or utilizing texture patterns. Realistic looking volume
renderings can be obtained by transferring the colors of a colored
volume such as the photographic Visible Human dataset (obtained
from actual photographs) to a volume of a different modality. In
this way, realistically colored volumes can be rendered, although
no actual color information is known \\

\textbf{Automation - - - }
Consulting the volume rendering and TF-related literature of the
last decade reveals a motivational statement that can be found in
many of the abstracts: Volume rendering has established itself as
a powerful visualization tool in many domains, but the necessary
design of TFs is a time consuming and tedious task. Consequently,
a significant amount of work is dedicated to the automatic and semiautomatic
generation of TFs. Based on the fundamental notions and
classifications of the TF concept, this section provides an overview
of the higher level aspects of TFs. This section also examines the
improvement of functionality and efficiency by introducing automatization
through data driven approaches as well as by utilizing user
knowledge encoded through interaction.\\

Instead of starting the TF design process anew for every new dataset,
Rezk-Salama et al. [RSHSG00] have proposed the reuse of existing,
manually designed TFs from previous similar datasets and adjusting
them by non-linear distortion to fit the new data. To perform the distortion,
the work has compared both the histograms of the datasets
and improved the initial results using Kindlmann and Durkin’s position
function [KD98]. Castro et al. [CKLG98] have suggested to
work with labeled components to further facilitate adjusting of presets
at this component level. Rezk-Salama et al. [RSKK06] later refined
their approach to utilize existing TFs. They have recommended
establishing a domain-specific semantic model of components in
the data and the manual definition of one or more 2D TF primitives
for each component. For a number of datasets, these primitives are
adjusted manually to account for the variation between datasets. The
adjustments are projected to one dimension using the first principal
component, and this single parameter is exposed to the novice user
as a slider.
In extension of their previous work on LiveSync, a system to synchronize
2D slice views and volumetric views of medical datasets,
Kohlmann et al. [KBKG08] have presented a new workflow and
interaction technique to aid the TF generation. As a starting point,
the user selects a point of interest (POI) in the slice view, and the
system refines and adapts TF presets based on statistical properties
derived from the selected POI. The system provides additional supportive
features, such as smart clipping, to reveal volume views that
are not occluded.\\

